CT respiratory motion synthesis using joint supervised and adversarial learning

Objective: Four-dimensional computed tomography (4DCT) imaging consists in reconstructing a CT acquisition into multiple phases to track internal organ and tumor motion. It is commonly used in radiotherapy treatment planning to establish planning target volumes. However, 4DCT increases protocol complexity, may not align with patient breathing during treatment, and lead to higher radiation delivery. Approach: In this study, we propose a deep synthesis method to generate pseudo respiratory CT phases from static images for motion-aware treatment planning. The model produces patient-specific deformation vector fields (DVFs) by conditioning synthesis on external patient surface-based estimation, mimicking respiratory monitoring devices. A key methodological contribution is to encourage DVF realism through supervised DVF training while using an adversarial term jointly not only on the warped image but also on the magnitude of the DVF itself. This way, we avoid excessive smoothness typically obtained through deep unsupervised learning, and encourage correlations with the respiratory amplitude. Main results: Performance is evaluated using real 4DCT acquisitions with smaller tumor volumes than previously reported. Results demonstrate for the first time that the generated pseudo-respiratory CT phases can capture organ and tumor motion with similar accuracy to repeated 4DCT scans of the same patient. Mean inter-scans tumor center-of-mass distances and Dice similarity coefficients were $1.97$mm and $0.63$, respectively, for real 4DCT phases and $2.35$mm and $0.71$ for synthetic phases, and compares favorably to a state-of-the-art technique (RMSim).

==> table.tex <==
% CHRU
\begin{table}
    \caption{\label{LungVolume_pvd} Lung volume variation and DSC with volume-based scalar on CHRU dataset.}
    \begin{indented}
        \item[]\begin{tabular}{@{}lllll}
        \br
        Lung Volume (ml)&Phase 2&Phase 3&Phase 4&Phase 5\\
        \mr
        Reference&3560.2±1305.1&3647.5±1312.3&3716.4±1321.9&3715.5±1334.8\\
        Generated&3556.8±1280.0&3627.5±1285.7&3677.1±1299.9&3678.1±1310.7\\
        \%Difference&1.3&1.4&1.8&1.7\\
        DSC &0.96±0.01&0.96±0.01&0.96±0.02&0.96±0.01\\
        \br
        \end{tabular}
    \end{indented}
\end{table}

\begin{table}
    \caption{\label{LungVolume_surface} Lung volume variation and DSC with surface-based scalar on CHRU dataset.}
    \begin{indented}
        \item[]\begin{tabular}{@{}lllll}
        \br
        Lung Volume (ml)&Phase 2&Phase 3&Phase 4&Phase 5\\
        \mr
        Reference&3560.2±1305.1&3647.5±1312.3&3716.4±1321.9&3715.5±1334.8\\
        Generated&3553.5±1275.0&3615.1±1275.0&3667.3±1311.1&3677.0±1332.2\\
        \%Difference&1.8&1.9&2.6&2.4\\
        DSC &0.95±0.01&0.95±0.01&0.94±0.02&0.94±0.01\\
        \br
        \end{tabular}
    \end{indented}
\end{table}

% TCIA 
\begin{table}
    \caption{\label{TCIA_ampli} Lung volume variation and DSC with volume-based scalar on TCIA dataset.}
    \begin{indented}
        \item[]\begin{tabular}{@{}lllll}
        \br
        Lung Volume (ml)&Phase 2&Phase 3&Phase 4&Phase 5\\
        \mr
        Reference&3506.1±1261.1&3601.7±1279.0&3754.6±1320.4&3919.7±1357.5\\
        Generated&3551.1±1258.3&3697.8±1282.8&3892.4±1298.2&4070.7±1318.2\\
        \%Difference&2.0&3.2&4.4&4.7\\
        DSC &0.96±0.02&0.95±0.01&0.95±0.02&0.95±0.03\\
        \br
        \end{tabular}
    \end{indented}
\end{table}

\begin{table}
    \caption{\label{TCIA_surface} Lung volume variation and DSC with surface-based scalar on TCIA dataset.}
    \begin{indented}
        \item[]\begin{tabular}{@{}lllll}
        \br
        Lung Volume (ml)&Phase 2&Phase 3&Phase 4&Phase 5\\
        \mr
        Reference&3506.1±1261.1&3601.7±1279.0&3754.6±1320.4&3919.7±1357.5\\
        Generated&3490.5±1235.1&3587.2±1279.3&3698.5±1306.9&3777.2±1347.7\\
        \%Difference&2.6&2.7&4.3&5.1\\
        DSC &0.96±0.01&0.95±0.02&0.95±0.02&0.95±0.02\\
        \br
        \end{tabular}
    \end{indented}
\end{table}


CHRU Surface	Phase 2	Phase 3	Phase 4	Phase 5	All
NCC_X	0.64±0.24	0.59±0.35	0.72±0.17	0.73±0.18	0.67±0.25
NCC_Y	0.75±0.42	0.82±0.30	0.85±0.13	0.86±0.14	0.82±0.28
NCC_Z	0.62±0.52	0.75±0.32	0.81±0.17	0.84±0.16	0.76±0.33
					
CHRU PVD	Phase 2	Phase 3	Phase 4	Phase 5	All
NCC_X	0.51±0.32	0.68±0.15	0.57±0.33	0.70±0.13	0.61±0.26
NCC_Y	0.78±0.34	0.82±0.31	0.85±0.22	0.90±0.08	0.84±0.26
NCC_Z	0.66±0.32	0.71±0.50	0.81±0.17	0.85±0.09	0.76±0.32
					
TCIA Surface old	Phase 2	Phase 3	Phase 4	Phase 5	All
NCC_X	0.12±0.30	0.36±0.36	0.55±0.34	0.68±0.26	0.43±0.38
NCC_Y	0.58±0.28	0.65±0.30	0.76±0.23	0.89±0.10	0.72±0.26
NCC_Z	0.56±0.34	0.53±0.50	0.73±0.42	0.89±0.11	0.68±0.40
					
TCIA PVD  old	Phase 2	Phase 3	Phase 4	Phase 5	All
NCC_X	0.17±0.31	0.38±0.39	0.61±0.37	0.70±0.31	0.46±0.40
NCC_Y	0.58±0.26	0.65±0.32	0.83±0.16	0.91±0.06	0.74±0.26
NCC_Z	0.60±0.40	0.68±0.40	0.81±0.18	0.88±0.13	0.74±0.32


\begin{table}
    \caption{\label{ncc} NCC of the DVFs.}
    \begin{indented}
        \item[]\begin{tabular}{@{}lllll}
        \br
        &CHRU& &TCIA& \\
        \mr
        &Surface&PVD&Surface&PVD\\
        $NCC_x$&0.67±0.25&0.61±0.26&0.43±0.38&0.46±0.40\\
        $NCC_y$&0.82±0.28&0.84±0.26&0.72±0.26&0.74±0.26\\
        $NCC_z$&0.76±0.33&0.76±0.32&0.68±0.40&0.74±0.32\\
        \br
        \end{tabular}
    \end{indented}
\end{table}
